Balance functions of charged hadron pairs $(\pi,K,p)\otimes (\pi,K,p)$ in Pb--Pb collisions at $\sqrt{s_{_{\rm NN}}} =$2.76 TeV

We present the first balance function (BF) measurement of charged hadron pairs $(\pi,K,p)\otimes (\pi,K,p)$ in Pb--Pb collisions at $\sqrt{s_{_{\rm NN}}} =$2.76 TeV. The BF measurements are carried out as two-dimensional (2D) differential correlators vs. the relative rapidity ($\Delta y$) and azimuthal angle ($\Delta\varphi$) of hadron pairs, and studied as a function of collision centrality. While the BF azimuthal widths of all pairs substantially decrease from peripheral to central collisions, the longitudinal widths exhibit mixed behaviors: BF of $\pi\pi$ and cross-species pairs narrow in more central collisions whereas those of $KK$ and $pp$ are found invariant with collision centrality. This dichotomy is qualitatively consistent with the presence of strong radial flow effects and the existence of two waves of quark production in relativistic heavy ion collisions. We additionally present first measurements of the BF integrals and find that hadron pairing probabilities are very different from single hadron ratios and feature minimal collision centrality dependence. Overall, the results presented provide new and challenging constraints for theoretical models of hadron production and transport in relativistic heavy ion collisions.

==> autobio.tex <==
\begin{center}
\textbf{AUTOBIOGRAPHICAL STATEMENT}
\end{center}
\noindent
\textbf{Name}:
\noindent
Name Here
\singlespacing

\noindent
\textbf{Education}:

\noindent
% bachelor's degree here, etc etc...

\noindent
%M.S. Physics, Some Other University, City, State, Year

\noindent
%\textbf{Professional Experience}:

\noindent
%Some Job, Dept. of Physics and Astronomy, Somewhere, Year

\noindent
\vphantom{a}

\noindent
\textbf{Publications}: 

\noindent
%[Reference]

\vphantom{a}

\doublespacing

%[Insert text here]

\noindent
\textbf{Presented Talks}:

\noindent
\textbf{Presented Posters}:


==> copyright.tex <==
% Use this if you intend to copyright your document

%\setcounter{page}{1} 
\newpage
\thispagestyle{empty}

\begin{center}
{\bf \copyright~COPYRIGHT BY \\
Jinjin Pan \\
2019 \\
All Rights Reserved \\
}
\end{center}

